Towards Robust Solvers for Nuclear Fusion Simulations Using JOREK: A Numerical Analysis Perspective

One of the most well-established codes for modeling non-linear Magnetohydrodynamics (MHD) for tokamak reactors is JOREK, which solves these equations with a B\'ezier surface based finite element method. This code produces a highly sparse but also very large linear system. The main solver behind the code uses the Generalized Minimum Residual Method (GMRES) with a physics-based preconditioner, but even with the preconditioner there are issues with memory and computation costs and the solver does not always converge well. This work contains the first thorough study of the mathematical properties of the underlying linear system. It enables us to diagnose and pinpoint the cause of hampered convergence. In particular, analyzing the spectral properties of the matrix and the preconditioned system with numerical linear algebra techniques, will open the door to research and investigate more performant solver strategies, such as projection methods.

==> chapters/addendum.tex <==
%!TEX root = ../main.tex

\appendix



\chapter*{Removed Sections}

Sections that I wrote fully or partially but am not likely to keep in the final document. Keeping around temporarily for posterity.


\section{Complex Formatting}

TODO: Ask JOREK about this, since it doesn't make sense to me how this would help with memory. Alternatively, remove this section.

When the preconditioner matrix has a certain amount of symmetry, it can be represented in a memory-efficient way with a complex-valued representation.

“In order to optimize performance of a direct solver we have exploited the idea of representing the preconditioner block- matrices in complex form. This reduces the memory consumption considerably and improve overall solve time. The transformation into complex format is only possible when the matrix has the appropriate symmetry structure.”



\section{Ideal MHD (Possibly remove this? Possibly irrelevant)}

Some assumptions can be relaxed. Ions weigh at least 3 orders of magnitude more than electrons (1,836x in the case of Hydrogen), and therefore travel far slower in a plasma. Since electrons travel throughout the plasma much faster, they react to disturbances much faster, driving a lot of plasma behavior. For example, a disturbance in the electric field will be balanced out by a displacement of the electrons, while the ions will remain relatively static. Owing to this significant difference in behavior, the "Ideal MHD" effectively treats electron reactivity as instant and the plasma as resistance-free. The resistivity term $\eta = 0$. Ohm's law goes from $\vec{E} + \vec{u} \times \vec{B} = \eta \vec{J} = 0$

\section{Ideal MHD}
parts:


\section{Full MHD}

TODO Read and draw from \cite{Full_MHD}
Hoelzl: "-> not used so much in production, since our reduced MHD model is doing a quite good job for most applications."

JOREK can also execute a full MHD model. However, this is not used much in production as the reduced model captures key physics very well under most conditions for less computation cost. For certain types of instabilities, the full MHD model is required.


\section{Numerical Stability}

A computer can only store and operate on numbers to a finite precision, so executing floating point operations on matrices naturally introduces “round-off errors,” typically on the order of the machine precision for floating point numbers ($10^{-16}$) or double precision numbers ($10^{-32}$) (TODO double check these). When a large number of operations build off of eachother, these tiny numbers can cascade into a significant source of error.


\section{From Research Proposal}
From the list: 
\begin{enumerate}
    \item Without changing the underlying model, can performance be improved by changing how the linear system is constructed? Is there a better way to discretize or to apply boundary conditions?
\end{enumerate}

\section{Alternate RMHD}

Since the perturbation of the toroidal magnetic field is of second order, but only enters into the equations of motion at third order (TODO: I don't understand this. Find this discussed in Franck), it can be neglected and we can take the toroidal magnetic field to be constant in time\cite{Franck_Reduced_MHD}, yielding. 
\begin{equation}
\mathbf{B}_\phi=\frac{F_0}{R} \mathbf{e}_\phi \text { and } \mathbf{B}_{p o l}=\frac{1}{R} \nabla \psi \times \mathbf{e}_\phi
\end{equation}

Expand from \cite{Krebs_Thesis}
TODO Expand on this from \cite{Hoelzl_2021}

"\cite{Franck_Reduced_MHD}The velocity field depends on the electrical potential in the poloidal plane and the parallel velocity (parallel to the magnetic field). It is given by
\begin{equation}
    \mathbf{v}=\mathbf{v}_{p o l}+\mathbf{v}_{\|}=-R \nabla u \times \mathbf{e}_\phi+v_{\|} \mathbf{B} .
\end{equation}
This choice comes from to the choice of the electrical potential $\mathbf{V}=\mathbf{F}_0 u$ with $\mathbf{E}=\nabla \mathbf{V}$ and the fact that the poloidal velocity is homogeneous to $\mathbf{E} \times \mathbf{B}$. This potential formulation allows to reduce the number of variables and filter the fast magnetosonic waves of the MHD for nearly incompressible flows. The full MHD system with all waves is a very stiff problem with restrictive CFL stability conditions and bad conditioning for the numerical methods. Consequently eliminating these waves allows to obtain a less stiff problem, which is easier to solve. To obtain the final reduced models we plug the potential formulations in the full MHD model and use projections to obtain the equations on $u$ and $v_{\|}$. For the equation on the electric potential we project by applying the operator $\mathbf{e}_\phi \cdot \nabla \times\left(R^2 \ldots\right)$ to the momentum equation. To obtain the equation on $\mathbf{v_{\|}}$we project by applying the operator $\mathbf{B} \cdot(\ldots)$ to the momentum equation."


The reduced model (see \cite{Franck_Reduced_MHD} for the full, exhaustive derivation) comes out to:
\begin{equation}
\left\{\begin{array}{l}
 \partial_t \frac{1}{R^2} \psi=\frac{1}{R}[\psi, u]+\frac{\eta}{R^2}\left(j+\frac{\partial_{\phi \phi} \psi}{R^2}\right)-\frac{1}{R^2} F_0 \partial_\phi u \\
 \nabla \cdot\left(\widehat{\rho} \nabla_{p o l} \partial_t u\right)-\nabla \cdot\left(\rho \partial_t\left(v_{\|} \nabla_{p o l} \psi\right)\right)=\frac{1}{2 R}\left[R^2\left|\nabla_{p o l} u\right|^2, \widehat{\rho}\right]+\frac{1}{R}\left[\widehat{\rho} R^2 w, u\right]-\frac{1}{R}\left[R^2, p\right]+\frac{1}{R}[\psi, j]-\frac{F_0}{R^2} \partial_\phi j \\
 +\nabla \cdot\left(\mu_{\perp} \nabla w\right)+\frac{1}{R}\left[\rho v_{\|}^2 j, \psi\right]+\frac{1}{R}\left[\rho v_{\|}\left(\nabla_{p o l} v_{\|} \cdot \nabla_{p o l} \psi\right), \psi\right]-\nabla \cdot\left(\widehat{\rho} \frac{F_0}{R^2} v_{\| \mid} \nabla_{p o l}\left(\partial_\phi u\right)\right) \\
 +\frac{1}{R}\left[\widehat{\rho}, v_{\|}\left(\nabla_{p o l} \psi \cdot \nabla_{p o l} u\right)\right]-\frac{1}{2 R}\left[\widehat{\rho}, v_{\|}^2\left|\mathbf{B}_{p o l}\right|^2\right]-\frac{1}{R}\left[\hat{\rho} v_{\|} w, \psi\right]+\frac{1}{R}\left[u, \widehat{\rho} v_{\|} j\right]+\frac{1}{R}\left[u, \widehat{\rho}\left(\nabla_{p o l} \psi \cdot \nabla_{p o l} v_{\|}\right)\right] \\
 +\frac{1}{R} \partial_Z\left(\widehat{\rho} \frac{F_0}{R^3} v_{\|} \partial_\phi\left(v_{\|} \partial_Z \psi\right)\right)+\frac{1}{R} \partial_R\left(\widehat{\rho} \frac{F_0}{R^3} v_{\|} \partial_\phi\left(v_{\|} \partial_R \psi\right)\right)-\frac{1}{R} \partial_Z\left(\widehat{\rho} \frac{F_0^2}{R^3} v_{\|}^2\right) \\
 w=\Delta_{p o l} u \\
 j=\Delta^* \psi \\
 \partial_t \rho=R[\rho, u]+2 \rho \partial_Z u-\frac{v_{\|} F_0}{R^2} \partial_\phi \rho-\frac{v_{\|}}{R}[\rho, \psi]-\frac{\rho}{R}\left[v_{\|}, \psi\right]-\frac{\rho F_0}{R^2} \partial_\phi v_{\|} \\
 \partial_t p=R[p, u]+2 \gamma p \partial_Z u-\frac{v_{\|} F_0}{R^2} \partial_\phi p-\frac{v_{\|}}{R}[p, \psi]-\frac{\gamma p}{R}\left[v_{\|}, \psi\right]-\frac{\gamma p F_0}{R^2} \partial_\phi v_{\|} \\
 \rho\left|\mathbf{B}^2\right| \partial_t v_{\|}+\rho v_{\| \mid} \frac{1}{R^2} \nabla_{p o l} \psi \cdot \nabla_{p o l}\left(\partial_t \psi\right)-\rho \nabla_{p o l} \psi \cdot \nabla_{p o l}\left(\partial_t u\right)=-\frac{1}{R}[p, \psi]-\frac{F_0}{R^2} \partial_\phi p+\frac{\rho}{R}\left[\psi, \frac{v_{\|}^2|\mathbf{B}|^2}{2}\right] \\
 -\frac{F_0}{R} \rho \partial_\phi\left(\frac{v_{\|}^2|\mathbf{B}|^2}{2 R}\right)-\frac{1}{2 R} \rho\left[R^2\left|\nabla_{p o l} u\right|^2, \psi\right]-\frac{\hat{\rho}}{R} w[\psi, u]-R \rho|\mathbf{B}|^2\left[u, v_{\|}\right]-R \rho v_{\|}\left[u, \frac{|\mathbf{B}|^2}{2}\right]+R \rho v_{\|}\left[u, \frac{\left|\mathbf{B}_{p o l}\right|^2}{2}\right] \\
 -\rho v_{\|} \frac{\Delta^* \psi}{R}[u, \psi]-\frac{\rho v_{\|}}{R}\left[\psi,\left(\nabla_{p o l} \psi \cdot \nabla_{p o l} u\right)\right]+\frac{\rho v_{\|} F_0}{R^2}\left(\nabla_{p o l} \psi \cdot \nabla_{p o l}\left(\partial_\phi u\right)\right)+\rho v_{\|} \frac{F_0^2}{R^2} \partial_Z u
\end{array}\right.
\end{equation}

Alternate alternate:


Two major assumptions are made \cite{Krebs_Thesis,Hoelzl_2021}:
\begin{enumerate}
    \item The time dependent part of the magnetic potential is dominated by the toroidal component. 
    \item The torodial component of the magnetic field dominates the poloidal component.
\end{enumerate}


------

Starting with the resistive MHD model, (TODO: Settle on a consistent notation) 
\begin{equation}
    \left\{\begin{array}{l}
    \partial_t \rho+\nabla \cdot(\rho \mathbf{v})=0 \\
    \rho \partial_t \mathbf{v}+\rho \mathbf{v} \cdot \nabla \mathbf{v}+\nabla p=\mathbf{J} \times \mathbf{B}+\nabla \cdot(\nu \nabla \mathbf{v}) \\
    \partial_t p+\mathbf{v} \cdot \nabla p+\gamma p \nabla \cdot \mathbf{v}=0 \\
    \partial_t \mathbf{B}=-\nabla \times \mathbf{E}=\nabla \times(\mathbf{v} \times \mathbf{B}-\eta \mathbf{J}) \\
    \nabla \times \mathbf{B}=\mathbf{J} \\
    \nabla \cdot \mathbf{B}=0
    \end{array}\right.
\end{equation}

\section{MHD stuff}

Our goal with this simulation is to watch the evolution of a plasma in time, so we formulate the MHD model as a set of equations to model the time evolution of our parameters: the magnetic potential $\mathbf{A}$, mean fluid velocity $\mathbf{V}$, total density $\rho$, and pressure $p$. We incorporate the magnetic vector potential defined by $\mathbf{B} = \nabla \times \mathbf{A} + F \nabla \phi$. 

(TODO: This is the "base MHD" model in the Hoelzl paper. Instead use maybe the Ideal and work from there to Reduced).
\begin{equation}
    \begin{aligned}
        \frac{\partial \mathbf{A}}{\partial t} & =-\mathbf{E}-\nabla \Phi \\
        \rho \frac{\partial \mathbf{V}}{\partial t}= & -\rho \mathbf{V} \cdot \nabla \mathbf{V}-\nabla p+\mathbf{J} \times \mathbf{B}+\nabla \cdot \underline{\tau}+\mathbf{S}_{\mathbf{V}} \\
        \frac{\partial \rho}{\partial t}= & -\nabla \cdot(\rho \mathbf{V})+\nabla \cdot(\underline{D} \nabla \rho)+S_\rho \\
        \frac{\partial p}{\partial t}= & -\mathbf{V} \cdot \nabla p-\gamma p \nabla \cdot \mathbf{V}+\nabla \cdot(\underline{\kappa} \nabla T) +(\gamma-1) \underline{\tau}: \nabla \mathbf{V}+S_p
    \end{aligned}
\end{equation}

Included in the above equation are the viscous stress tensor $\underline{\tau}$, the particle diffusion tensor $
\underline{D}$, the heat diffusion tensor $\underline{\kappa}$, and the ratio of specific heats $\gamma$ (usually 5/3). S-terms are sources for volume, particles, and pressure

\section{Weak Form}


"Following the representation of A and V in the basis $(\mathbf{e}_R, \mathbf{e}_Z , \mathbf{e}_{\psi})$, and $(\mathbf{e}_R, \mathbf{e}_Z , \mathbf{B})$ respectively, the basis for the
vector test function $\mathbf{V}$ and $\mathbf{A}$ in the weak formulation"

\begin{equation}
\begin{aligned}
\mathbf{A} & =A_R \mathbf{e}_R+A_Z \mathbf{e}_Z+\frac{1}{R} A_3 \mathbf{e}_{\varphi} \\
\mathbf{V} & =V_R \mathbf{e}_R+V_Z \mathbf{e}_Z+V_{\|} \mathbf{B} \\
\mathbf{A}^{\star} & =a^*\left(\mathbf{e}_R, \mathbf{e}_Z, \mathbf{e}_{\varphi}\right) \\
\mathbf{V}^{\star} & =v^*\left(\mathbf{e}_R, \mathbf{e}_Z, \mathbf{B}\right)
\end{aligned}
\end{equation}

"where $a^*$ and $v^*$ represent the scalar test functions."

\section{Preconditioned GMRES}

For GMRES, left, right, and split preconditioners can all be used. Unless A is highly symmetric or M is ill-conditioned, there is little difference between these forms in practice. The operators they produce ($\mathbf{M}^{-1}\mathbf{A},\; \mathbf{AM}^{-1},\;\text{and }\mathbf{L}^{-1}\mathbf{AU}^{-1}$) all have the same spectra, but as discussed, GMRES convergence is not purely due to spectrum. Eigenvalues do not always govern convergence and so these can have very different performance\cite{Saad_96}. However in practice, the spectrum often drives convergence

The approximate solution obtained for GMRES by left or right (TODO: Expand why/when to use left/right) conditioning is 
\begin{equation}
    x_m = x_0 + s_{m-1}(\mathbf{M}^{-1}\mathbf{A})z_0 = x_0 + \mathbf{M}^{-1}s_{m-1}(\mathbf{AM}^{-1})r_0
\end{equation}
where $z_0 = \mathbf{M}^{-1}r_0$ and $s_{m-1}$ is a polynomial of degree m that minimizes the residual norm $||b - \mathbf{A}x_m||_2$ if preconditioned from the right, and $||\mathbf{M}^{-1}(b-\mathbf{A}x_m)||_2$ if preconditioned from the left.

The convergence behavior ... TODO


\section{BiCGSTAB Convergence}

BiCGSTAB can converge poorly if for many consecutive steps, the angle between the residual $r$ and $\mathbf{A}r$ is larger than 45 degrees. No breakdown or near-breakdown of convergence will occur if the angle between the Krylov subspace and the "shadow" Krylov subspace ...

---

the machine error is bounded by
\begin{equation}
    \left|\epsilon_k\right| \leq 1.0 \ln \bar{\xi} \frac{\left\|r_k\right\|\left\|\psi_k\left(A^T\right) \tilde{r}_0\right\|}{\left|\left(r_k, \psi_k\left(A^T\right) \tilde{r}_0\right)\right|} \leq \frac{1.0 \ln \bar{\xi}}{\hat{\rho}_k}
\end{equation}

where $\bar{\xi}$ is the relative precision and n is the number of dimensions.

$\psi_k$ is a sequence of polynomials of degree k, which can form a basis of the Krylov subspace $K(A^t, r_0$ as $\psi_0\left(A^T\right) \tilde{r}_0, \ldots, \psi_{k-1}\left(A^T\right) \tilde{r}_0$.

----


\begin{colbox}{blue!10}
\end{colbox}

==> chapters/analysis.tex <==
%!TEX root = ../main.tex

% \chapter{Research and Analysis}




==> chapters/failed.tex <==
%!TEX root = ../main.tex

\chapter{Failed Attempts}

\section{Python Implementation}

TODO: Discuss the Python implementation
Python/Numpy/Scipy used a different direct solver, and gave me different behavior. Theory is that it's possible the system is so incredibly poorly conditioned that this small difference may have resulted in different behavior.

\section{Explicit Preconditioner}

TODO: Discuss failure to generate explicit preconditioners, and some of our theory on getting around this -- Given spectral extrema on our $M$ preconditioner blocks, using Gershgorin's theorem to draw spectral bounds on the $M^{-1}A$ system.

\section{TODO}

==> chapters/research_plan.tex <==
%!TEX root = ../main.tex

\section{Research Plan}

For some settings, the JOREK team sees poor convergence when trying to solve the linear system. The goal of this project is to analyze JOREK's linear system and solver so as to drive better overall performance. In particular, the team behind JOREK has asked us to:
\begin{enumerate}
    \item Understand what limits the solver's convergence. What causes the bad convergence they occasionally see. Is this driven by e.g. a setting in the physics model or spatial feature? Is there a way to predict how a given run will perform without running the whole solver?

    \item How does this behavior link to their numerical solvers? For what conditions does GMRES perform better or worse than other methods such as BICGSTAB?
    
    \item Can we improve the preconditioner? Is there anything we can do to improve on memory usage, computation cost, or convergence? Is there anything about the matrix construction or physics model that could inform the construction of the preconditioner?
\end{enumerate}

\section{Research Plan}

The JOREK team sends us data in the form of linear systems. These are systems and associated preconditioners, in a sparse format, and encoded in the HDF5 file format. 

By studying several systems with a range of convergence behavior, we hope to understand and isolate features that negatively impact solver convergence. We will analyze these and determine if there is anything particular about them that leads to poor performance. Is the problem ill-conditioned? Does it have a particular spectrum that leads to poor performance for certain approaches?

Then we will attempt to see if there are any "easy wins" in terms of solving or preconditioning these problems. Is there a preconditioner we could use to solve these with any generality? The literature suggests other potential preconditioners for MHD, such as \cite{Ma_Preconditioners_MHD,Laakmann_2022}. Are there any minor features to the matrix that can be adjusted? Are there other solvers we could use, such as BICGSTAB or variants of GMRES that would be preferred in some cases? For example, some GMRES algorithms that incorporate spectral information on restarts can overcome stalling or improve convergence in certain cases \cite{Baker_2004, Morgan_Restarted_GMRES}.



==> chapters/results.tex <==
%!TEX root = ../main.tex

\chapter{Results}

